VARADE: a Variational-based AutoRegressive model for Anomaly Detection on the Edge

Detecting complex anomalies on massive amounts of data is a crucial task in Industry 4.0, best addressed by deep learning. However, available solutions are computationally demanding, requiring cloud architectures prone to latency and bandwidth issues. This work presents VARADE, a novel solution implementing a light autoregressive framework based on variational inference, which is best suited for real-time execution on the edge. The proposed approach was validated on a robotic arm, part of a pilot production line, and compared with several state-of-the-art algorithms, obtaining the best trade-off between anomaly detection accuracy, power consumption and inference frequency on two different edge platforms.

==> tables/data_stream2.tex <==
\begin{tabular}{l||l|l}

Channel name                             & Unit               & Description                                \\ 
\hline \hline
action ID                                       & -                  & Robot action ID                            \\

apparent\_power                              & VA                 & Apparent power                             \\
current                                      & A                  & Current                                    \\
frequency                                    & Hz                 & Frequency                                  \\
phase\_angle                                 & degree             & Phase angle                                \\
power                                        & W                  & Power                                      \\
power\_factor                                & -                  & Power factor                               \\
reactive\_power                              & VAr                & Reactive power                             \\
voltage                                      & V                  & Voltage                                    \\
sensor\_id\_<X>\_AccX                        & m/s$^2$            & X-axis acceleration                        \\
sensor\_id\_<X>\_AccY                        & m/s$^2$            & Y-axis acceleration                        \\
sensor\_id\_<X>\_AccZ                        & m/s$^2$            & Z-axis acceleration                        \\
sensor\_id\_<X>\_GyroX                       & deg/s              & X-axis angular velocity                    \\
sensor\_id\_<X>\_GyroY                       & deg/s              & Y-axis angular velocity                    \\
sensor\_id\_<X>\_GyroZ                       & deg/s              & Z-axis angular velocity                    \\
sensor\_id\_<X>\_q1                          & -                  & Quaternion orientation comp. 1             \\
sensor\_id\_<X>\_q2                          & -                  & Quaternion orientation comp. 2             \\
sensor\_id\_<X>\_q3                          & -                  & Quaternion orientation comp. 3             \\
sensor\_id\_<X>\_q4                          & -                  & Quaternion orientation comp. 4             \\
sensor\_id\_<X>\_temp                        & $^\circ$C          & Temperature                                \\
% anomaly                                      & -                  & Anomaly label                              \\                  
\hline
\end{tabular}
